Quantum Information Scrambling, Chaos, Sensitivity, and Emergent State Designs

Understanding quantum chaos is of profound theoretical interest and carries significant implications for various applications, from condensed matter physics to quantum error correction. Recently, out-of-time ordered correlators (OTOCs) have emerged as a powerful tool to quantify quantum chaos. For a given quantum system, the OTOCs measure incompatibility between an operator evolved in the Heisenberg picture and an unevolved operator. In the first part of this thesis, we employ OTOCs to study the dynamical sensitivity of a perturbed non-Komogorov-Arnold-Moser (non-KAM) system in the quantum limit as the parameter that characterizes the $\textit{resonance}$ condition is slowly varied. For this purpose, we consider a quantized kicked harmonic oscillator (KHO) model that displays stochastic webs in the phase space. The OTOC analysis is followed by a study of quantum Fisher information (QFI) at the resonances and a comparison with the non-resonance cases. We shall show that scaling of the QFI in time is enhanced at the resonances, making the dynamics of the non-KAM systems good candidates for quantum sensing. In the following chapter, we study the OTOCs in a bipartite system of kicked coupled tops with a special focus on the mixed phase space OTOC dynamics. The last part of the thesis is devoted to the study of the emergence of quantum state designs as a signature of quantum chaos and the role of symmetries in this phenomenon. Recently proposed projected ensemble framework utilizes quantum chaos as a resource to construct approximate higher-order state designs. Despite being ubiquitous, the effects of symmetries on the emergence of quantum state designs remain under-explored. We thoroughly investigate this by demonstrating the interplay between symmetries and measurements in constructing approximate state designs. Finally, we outline a few open directions relevant to the current thesis.

==> chap-lists.tex <==
\chapter{Itemized Lists and Quotes}

Itemized lists work as one would expect. They are properly line-spaced. Refer
to the tutorial for more details. In general, it is better to start a new 
paragraph (i.e. place a blank line in the source file) at the start of a new 
enumerate block. This ensures that the line-spacing options are activated 
correctly.

Line spacing of items in the list and the spacing of the list with respect to
the surrounding textual matter is set as per the institute guidelines.

\section{Unnumbered lists}
These are the standard \textquote{bulleted} lists that one is familiar with.
\begin{enumerate}[blt]
    \item this
    \item is
    \item a bulletted
    \item list
\end{enumerate}

this is the next paragraph

\begin{enumerate}[dmd]
    \item this
    \item is
    \item a dashed
    \item list
\end{enumerate}

and this is the next paragraph

\begin{enumerate}[dsh]
    \item this
    \item[$\blacksquare$] is
    \item[\textbullet] a mixed
    \item list
\end{enumerate}

and this is the next paragraph

\begin{enumerate}[str]
    \item this
    \item is
    \item[\textbullet] a mixed
    \item list
\end{enumerate}

and this is the next paragraph

\begin{enumerate}[sqr]
    \item this
    \item is
    \item square
    \item list
\end{enumerate}

and this is the next paragraph 

\begin{enumerate}[bsq]
    \item this
    \item is
    \item square
    \item list
\end{enumerate}

\section{Numbered lists}
These are the standard numbered lists that one might be familiar with.
\begin{enumerate}
    \item this
    \item is a
    \item numbered
    \item list
\end{enumerate}

this is the next paragraph

\begin{enumerate}[i.]
    \item this
    \item is a
    \item roman-numbered
    \item list
\end{enumerate}


this is the next paragraph

\begin{enumerate}[I{]}]
    \item this
    \item is a
    \item capitalized roman-numbered
    \item list
\end{enumerate}

this is the next paragraph

\begin{enumerate}[a)]
    \item this
    \item is an
    \item alphabetical
    \item list
\end{enumerate}

this is the next paragraph

\begin{enumerate}[A\}]
    \item this
    \item is the
    \item last
    \item This is what that author said and it is rather important. That is the
    reason I am quoting the entire passage here for reference and completeness
    \begin{enumerate}
        \item This is what that author said and it is rather important. That is
the reason I am quoting the entire passage here for reference and completeness
        \item  This is what that author said and it is rather important. That is
the reason I am quoting the entire passage here for reference and completeness
    \end{enumerate}
\end{enumerate}

Note that one can nest lists as well as shown above

\section{More complex lists made easy}
\begin{enumerate}[{Step rsc{]}}, leftmargin=2cm]
    \item reflect over the research done
    \item review ones notes, writings, lab journal and research articles
    \item stop overthinking and/or procrastinating
    \item start writing
    \item realize that there is much to do
    \begin{enumerate}[{i\}}]
        \item fear not
        \item[$\star$] persevere
        \item continue writing
    \end{enumerate}
    \item success!
\end{enumerate}


\section{Quotes}

Very useful for quoting text from other works. See the tutorial for more
details and references.

An inline-quote, one that is along with the main material is placed like this
\textquote{this is a quote}. Sometimes we want to mention the author as well
\textquote[Author of the quote]{this is what that author wrote}

Sometimes, it is better to quote larger passages of text in the display mode
like this

\begin{displayquote}
This is what that author said and it is rather important. That is the reason I
am quoting the entire passage here for reference and completeness
\end{displayquote}

this is the next paragraph. By specifiying the optional argumnet, the author
name can be set as well:

\begin{displayquote}[Authorname]
This is what that author said and it is rather important. That is the reason I
am quoting the entire passage here for reference and completeness
\end{displayquote}

\section{Footnotes}
One might find the need to include some relevant contextual information in the
material but find it unneccessarily intrusive to do so in the running text
matter itself. In such cases, or whenever else the author feels the need to do
so, a footnote may be deployed thus \footnote{see, this is the footnote I was
talking about. It is spaced appropriately. Best to use these sparingly since
they detract from the general flow of the document. Some thoughtful
restructuring of the material can help reduce the need for footnotes}

==> glossary.tex <==
\iffalse
\newglossaryentry
    {latex}
    {
        name        = {\LaTeX},
        description = {{\LaTeX} is a popular macro package for document preparation},
    }

\newglossaryentry
    {math}
    {
        name        = {Mathematics},
        description = {A very versatile language},
    }

\newglossaryentry
    {phy}
    {
        name        = {Physics},
        description = {Trying to understand the world by describing it using mathematics},
    }

\newglossaryentry
    {csprog}
    {
        name        = {Computer Science and Programming\ \ },
        description = {An art form that is commonly associated with bringing silicon to life},
    }

\newglossaryentry
    {engg}
    {
        name        = {Engineering},
        description = {A popular scientific discipline},
    }


\fi


\newacronym{OTOCs} {OTOCs} {Out-of-time-ordered correlators}
\newacronym{KAM} {KAM} {Kolmogorov-Arnold-Moser}
\newacronym{RMT} {RMT} {Random matrix theory}
\newacronym{CUE} {CUE} {Circular unitary ensemble}
\newacronym{GUE} {GUE} {Gaussian unitary ensemble}
\newacronym{COE} {COE} {Circular orthogonal ensemble}
\newacronym{GOE} {GOE} {Gaussian orthogonal ensemble}
\newacronym{CSE} {CSE} {Circular symplectic ensemble}
\newacronym{GSE} {GSE} {Gaussian symplectic ensemble}
\newacronym{bgs} {BGS} {Bohigas-Giannoni-Schmit}
\newacronym{TI} {TI} {Translation invariant}
\newacronym{ETH} {ETH} {eigenstate thermalization hypothesis}
\newacronym{PBC} {PBC} {Periodic boundary conditions}
\newacronym{OBC} {OBC} {Open boundary conditions}
\newacronym{KHO} {KHO} {Kicked harmonic oscillator}
\newacronym{KCT} {KCT} {Kicked coupled tops}
\newacronym{LE} {LE} {Lyapunov exponent}
